The GitHub Development Workflow Automation Ecosystems

Large-scale software development has become a highly collaborative and geographically distributed endeavour, especially in open-source software development ecosystems and their associated developer communities. It has given rise to modern development processes (e.g., pull-based development) that involve a wide range of activities such as issue and bug handling, code reviewing, coding, testing, and deployment. These often very effort-intensive activities are supported by a wide variety of tools such as version control systems, bug and issue trackers, code reviewing systems, code quality analysis tools, test automation, dependency management, and vulnerability detection tools. To reduce the complexity of the collaborative development process, many of the repetitive human activities that are part of the development workflow are being automated by CI/CD tools that help to increase the productivity and quality of software projects. Social coding platforms aim to integrate all this tooling and workflow automation in a single encompassing environment. These social coding platforms gave rise to the emergence of development bots, facilitating the integration with external CI/CD tools and enabling the automation of many other development-related tasks. GitHub, the most popular social coding platform, has introduced GitHub Actions to automate workflows in its hosted software development repositories since November 2019. This chapter explores the ecosystems of development bots and GitHub Actions and their interconnection. It provides an extensive survey of the state-of-the-art in this domain, discusses the opportunities and threats that these ecosystems entail, and reports on the challenges and future perspectives for researchers as well as software practitioners.

==> book/acknowledgement.tex <==
%%%%%%%%%%%%%%%%%%%%%%acknow.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample acknowledgement chapter
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\extrachap{Acknowledgements}

Use the template \emph{acknow.tex} together with the document class SVMono (monograph-type books) or SVMult (edited books) if you prefer to set your acknowledgement section as a separate chapter instead of including it as last part of your preface.



==> book/acronym.tex <==
%%%%%%%%%%%%%%%%%%%%%%acronym.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample list of acronyms
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer Nature%%%%%%%%%%%%%%%%%%%%%%%%%%

\extrachap{Acronyms}

%Lists of abbreviations\index{acronyms, list of}, symbols\index{symbols, list of} and the like are easily formatted with the help of the Springer Nature enhanced \verb|description|\quad~environment.

\begin{description}%[CABR]

\item[A]~\\
\verb|ACM|\quad~Association for Computing and Machinery -- See \url{www.acm.org}

\verb|API|\quad~Application Programming Interface

\verb|AI|\quad~Artificial Intelligence

\verb|AST|\quad~Abstract Syntax Tree

\verb|AUG|\quad~API Usage Graph -- See \chap{SLU}.

\verb|AWS|\quad~Amazon Web Services -- A cloud computing platform proposed by Amazon. See \url{aws.amazon.com}

\item[B]~\\
\verb|BPMN|\quad~Business Process Modeling Notation


\item[C]~\\
\verb|CE|\quad~Collateral Evolution -- See \chap{COL}.

\verb|CHAOSS|\quad~Community Health Analytics in Open Source Software -- See \url{chaoss.community}

\verb|CI|\quad~Continuous Integration -- See \verb|CI/CD|.

\verb|CI/CD|\quad~Continuous Integration, Deployment and Delivery

\verb|CNN|\quad~Convolutional Neural Network -- A specific kind of Neural Network. %(\verb|NN|). 

\verb|CPS|\quad~Cyber-Physical System

\verb|CSP|\quad~Constraint Satisfaction Problem

\verb|CSV|\quad~Comma Separated Values -- A very simple data format.


\item[D]~\\
\verb|DAO|\quad~Data Access Object

\verb|DAG|\quad~Directed Acyclic Graph

\verb|DB|\quad~Database

\verb|DBMS|\quad~Database Management System

\verb|DE&I|\quad~Diversity, Equity and Inclusion -- A set of principles to build inclusive and welcoming workspaces and environments for less privileged individuals or organisations.

\verb|DL|\quad~Deep Learning -- A branch of Artificial Intelligence %(\verb|AI|)
 focused on developing algorithms and applications based on Neural Networks. %(\verb|NN|). 

\verb|DSL|\quad~Domain-Specific Language

\verb|DT|\quad~Decision Tree -- A specific kind of \emph{supervised} machine learning %(\verb|ML|) 
where the classifier is modeled as a tree.


\item[E]~\\
\verb|EIC|\quad~Error-Inducing Change

\verb|EMF|\quad~Eclipse Modeling Framework

\verb|EMR|\quad~Electronic Medical Record

\verb|EOSC|\quad~European Open Science Cloud -- a European Commission initiative aiming at developing an infrastructure providing its users with services promoting open science practices. See \url{eosc-portal.eu}


\item[F]~\\
\verb|FAIR|\quad~Findable, Accessible, Interoperable, Reusable -- Four guiding principles for scientific data management.

\verb|FFNN|\quad~Feed-Forward Neural Network -- A specific kind of Neural Network.% (\verb|NN|). 

\verb|FK|\quad~Foreign Key -- A kind of constraint that is frequently used in relational databases.

\verb|FL|\quad~Federated Learning -- A decentralised form of machine learning %(\verb|ML|)
that can be used to train models on decentralised data.

\verb|FOSS|\quad~Free Open Source Software -- See \verb|OSS|.

\verb|FP|\quad~False Positive

\verb|FSF|\quad~Free Software Foundation -- See \url{www.fsf.org}

\verb|FUSE|~\quad~Filesystem in User SpacE -- See \chap{SWH}.


\item[G]~\\
\verb|GDBT|\quad~Gradient Boosted Decision Tree -- A specific kind of Decision Tree. %(\verb|DT|).

\verb|GDPR|\quad~General Data Protection Regulation -- A data protection law imposed by the European Union.

\verb|GK|\quad~Graph Kernel -- A method to compute the internal weights of a graph neural network. See \chap{MDE}.

\verb|GNN|\quad~Graph Neural Network -- A specific kind of Neural Network. %(\verb|NN|). 

\verb|GNU|\quad~Recurvise acronym for GNU's Not Unix

\verb|GraphQL|\quad~Graph Query Language -- A query language for building flexible, efficient and powerful \verb|API|s.

\item[H]~\\
\verb|HQL|\quad~Hibernate Query Language -- An \verb|SQL|-like query language for Hibernate.


\item[I]~\\
\verb|IaC|\quad~Infrastructure as Code

\verb|ICSME|\quad~International Conference on Software Maintenance and Evolution -- The name of an annual scientific \verb|IEEE| conference.

\verb|IDE|\quad~Integrated Development Environment

\verb|IEEE|\quad~Institute of Electrical and Electronics Engineers -- See \url{www.ieee.org}

\verb|INRIA|\quad~Institut National de Recherche en Informatique et en Automatique -- French National Institute for Research in Computer Science and Control

\verb|IT|\quad~Information Technology


\item[J]~\\
\verb|JDBC|\quad~Java Database Connectivity

\verb|JDK|\quad~Java Development Kit

\verb|JPA|\quad~Jakarta Persistence API (formerly known as Java Persistence API) -- A Java specification to manage object-relational mappings (\verb|ORM|) between Java applications and a relational database.

\verb|JSON|\quad~JavaScript Object Notation -- A human-readable data serialisation language and file format, just like \verb|XML| and \verb|YAML|.


\item[L]~\\
\verb|LOC|\quad~Lines of Code

\verb|LR|\quad~Linear Regression

\verb|LSTM|\quad~Long Short-Term Memory -- A specific kind of Recurrent Neural Network. %(\verb|RNN|). 


\item[M]~\\
%\verb|MDD|\quad~Model-Driven Development -- See \verb|MDE|

\verb|MDE|\quad~Model-Driven (Software) Engineering

\verb|ML|\quad~Machine Learning -- A branch of computer science that uses algorithms trained on data to produce models that can perform complex tasks such as analysing, reasoning and learning.

\verb|MOF|\quad~Meta-Object Facility -- A domain-specific modeling language proposed by the \verb|OMG| for specifying metamodels for a variety of modeling languages (including \verb|UML|) to be used in the context of \emph{software engineering} (\ie for specifying, analysing, designing, verifying and validating software systems).

\verb|MSR|\quad~Mining Software Repositories -- The name of an annual scientific \verb|IEEE| conference.


\item[N]~\\
\verb|NATO|\quad~North Atlantic Treaty Organization -- See \url{www.nato.int}

\verb|NB|\quad~Na\"ive Bayesian -- A specific kind of \emph{supervised} machine learning %(\verb|ML|) 
technique.

\verb|NIST|\quad~National Institute of Standards and Technology -- Part of the US Department of Commerce. See \url{www.nist.gov}

\verb|NLP|\quad~Natural Language Processing -- A branch on the intersection of computer science and computational linguistics focused understanding, interpreting and manipultating \emph{natural} (\ie \emph{human}) language.

\verb|NN|\quad~Neural Network -- A computational technique in the area of Artificial Intelligence (\verb|AI|) that is at the heart of Deep Learning (\verb|DL|) algorithms.

\verb|NoSQL|\quad~Not Only SQL or non-SQL -- An category of database management systems %(\verb|DBMS|)
 that enable storing and querying data outside the traditional relational \verb|DBMS| that rely on \verb|SQL| as a query language.

\verb|NVD|\quad~National Vulnerability Database -- A software security vulnerability database maintained by \verb|NIST|. See \url{nvd.nist.gov}

\item[O]~\\
\verb|OCI|\quad~Oracle Cloud Infrastructure

\verb|OCL|\quad~Object Constraint Language -- A query and constraint language proposed by the \verb|OMG| to be used to query or express constraints over models (\eg \verb|UML| and \verb|SysML|) or metamodels (\eg \verb|MOF|).

\verb|OMG|\quad~Object Management Group -- An international non-profit consortium focused on developing technology standards such as \verb|UML|, \verb|SysML| and many more.

\verb|ORM|\quad~Object Relational Mapping -- A technique or framework used to simplify the mapping and translation between object-oriented programs and relational databases.

\verb|OS|\quad~Operating System

\verb|OSI|\quad~Open Source Initiative -- See \url{opensource.org}

\verb|OSS|\quad~Open Source Software


\item[P]~\\
\verb|PDG|\quad~Program Dependency Graph

\verb|PNG|\quad~Portable Network Graphic -- A data format for image files.

\verb|PR|\quad~Pull Request


\item[Q]~\\
\verb|QA|\quad~Quality Assurance

\verb|Q&A|\quad~Question and Answer


\item[R]~\\
\verb|RAM|\quad~Random Access Memory

\verb|REST|\quad~Representational State Transfer -- An architectural style for allowing computer systems to communicate with each other.

\verb|RF|\quad~Random Forest -- A specific kind of  supervised machine learning %(\verb|ML|)
technique.

\verb|RL|\quad~Reinforcement Learning -- One of the three machine learning paradigms, alongside \emph{supervised} and \emph{unsupervised} learning.

\verb|RNN|\quad~Recurrent Neural Network -- A specific kind of Neural Network. %(\verb|NN|). 

\verb|ROS|\quad~Robot Operating System -- See \url{www.ros.org}

\verb|RTM|\quad~Relational Topic Model


\item[S]~\\
\verb|SATD|\quad~Self-Admitted Technical Debt -- A specific kind of Technical Debt. %(\verb|TD|).

\verb|SBSE|\quad~Search-Based Software Engineering

\verb|SE|\quad~Software Engineering

\verb|SemVer|\quad~Semantic Versioning -- See \url{semver.org}

\verb|SHA1|\quad~Secure Hash Algorithm 1 -- A well-known cryptographic hash algorithm.

\verb|SPDX|\quad~Software Package Data Exchange -- An open standard for software bill of materials. See \url{spdx.dev}

\verb|SQL|\quad~Structured Query Language -- A language used to query data stored in a relational database.

\verb|SSD|\quad~Social Semantic Diversity

\verb|SVG|\quad~Scalable Vector Graphic -- A data format for image files.

\verb|SVM|\quad~Support Vector Machines -- A specific kind of \emph{supervised} machine learning %(\verb|ML|)
technique.

\verb|SWH|~\quad~Software Heritage -- See \chap{SWH}

\verb|SWHID|~\quad~Software Heritage Persistent Identifier -- See \chap{SWH}

\verb|SysML|\quad~Systems Modeling Language -- A modeling language proposed by the \verb|OMG| to be used in the context of \emph{systems engineering} (\ie specifying, analysing, designing, verifying and validating systems).


\item[T]~\\
\verb|TD|\quad~Technical Debt

\verb|TP|\quad~True Positive


\item[U]~\\
\verb|UML|\quad~Unified Modeling Language -- A modeling language proposed by the \verb|OMG| to be used in the context of \emph{software engineering} (\ie specifying, analysing, designing, verifying and validating software systems).

\verb|UNESCO|\quad~United Nations Educational, Scientific and Cultural Organization -- See \url{www.unesco.org}

\verb|URI|\quad~Uniform Resource Identifier

\verb|URL|\quad~Uniform Resource Locator


\item[V]~\\
\verb|VCS|\quad~Version Control System

\item[X]~\\
\verb|XML|\quad~eXtensible Markup Language -- A human-readable data serialisation language and file format, just like \verb|YAML| and \verb|JSON|.

\verb|XP|\quad~eXtreme Programming -- One of the many agile software development methodologies.


\item[Y]~\\
\verb|YAML|\quad~Recursive acronym for YAML Ain't Markup Language -- A human-readable data serialisation language and file format, just like \verb|XML| and \verb|JSON|.

\end{description}


==> book/contriblist.tex <==
%%%%%%%%%%%%%%%%%%%%clist.tex %%%%%%%%%%%%%%%%%%%%%%%%
%                                                    
% sample list of contributors and their addresses    
%                                                    
% Use this file as a template for your own input.    
%                                                    
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%
\contributors

\begin{thecontriblist}
%A
Mehrdad {\bf Abdi}
\at AnSyMo, Universiteit Antwerpen\\
Middelheimlaan 1, 2020 Antwerpen, Belgium\\
\email{newmrd@gmail.com}
\and
%B
John {\bf Businge}
\at Evol, University of Nevada Las Vegas\\
Maryland Pkwy, Las Vegas, 89154, U.S.A\\
\email{john.businge@unlv.edu}\\
\url{https://www.unlv.edu/people/john-businge}
\and
%C
Anthony {\bf Cleve}
\at Facult\'e d’informatique, Universit\'e de Namur\\
rue Grandgagnage 21, 5000 Namur, Belgium\\
\email{anthony.cleve@unamur.be}\\
\url{https://directory.unamur.be/staff/acleve}
\and
%D
Serge {\bf Demeyer}
\at AnSyMo, Universiteit Antwerpen\\
Middelheimlaan 1, 2020 Antwerpen, Belgium\\
FlandersMake\@UAntwerpen,\\
\email{serge.demeyer@uantwerpen.be}\\
\url{https://www.uantwerpen.be/en/staff/serge-demeyer/}
\and
Alexandre {\bf Decan}
\at Software Engineering Lab, University of Mons\\
Avenue Maistriau 15, 7000 Mons, Belgium\\
\email{alexandre.decan@umons.ac.be}\\
\url{https://decan.lexpage.net}
\and
Coen {\bf De Roover}
\at Software Languages Lab, Vrije Universiteit Brussel\\
Pleinlaan 2, 1050 Elsene, Belgium\\
\email{coen.de.roover@vub.be}\\
\url{http://soft.vub.ac.be/~cderoove}
\and
Roberto {\bf Di Cosmo}
\at Software Heritage -- INRIA and Université de Paris Cité\\
2, Rue Simone Iff, CS 42112, 75589 Paris Cedex 12, France\\
\email{roberto@dicosmo.org}\\
\url{https://dicosmo.org}
\and
Davide {\bf Di Ruscio}
\at University of L'Aquila\\
Via Vetoio snc, L'Aquila, Italy\\
\email{davide.diruscio@univaq.it}\\
\url{https://www.disim.univaq.it/DavideDiRuscio}
\and
%I
Katsuro {\bf Inoue}
\at Nanzan University\\
18 Yamazato-cho, Showa-ku, Nagoya, Japan\\
\email{inoue599@nanzan-u.ac.jp}\\
\url{https://sel.ist.osaka-u.ac.jp/people/inoue}
\and
%K
Raula Gaikovina {\bf Kula}
\at Nara Institute of Science and Technology\\
8916-5 Takayama, Ikoma, Nara, Japan\\
\email{raula-k@is.naist.jp}\\
\url{https://raux.github.io}
\and
%L
Michele {\bf Lanza}
\at Software Institute, Università della Svizzera italiana\\
Via G. Buffi 13, 6900 Lugano, Switzerland\\
\email{michele.lanza@usi.ch}\\
\url{https://www.inf.usi.ch/lanza}
\and
David {\bf Lo}
\at Singapore Management University\\
80 Stamford Road, Singapore 178902\\
\email{davidlo@smu.edu.sg}\\
\url{http://www.mysmu.edu/faculty/davidlo}
\and
%M
Tom {\bf Mens}
\at Software Engineering Lab, University of Mons\\
Avenue Maistriau 15, 7000 Mons, Belgium\\
\email{tom.mens@umons.ac.be}\\
\url{https://staff.umons.ac.be/tom.mens}
\and
%N
Csaba {\bf Nagy}
\at Software Institute, Università della Svizzera italiana\\
Via G. Buffi 13, 6900 Lugano, Switzerland\\
\email{csaba.nagy@usi.ch}\\
\url{https://csnagy.github.io}
\and
%
Phuong T. {\bf Nguyen}
\at University of L'Aquila\\
Via Vetoio snc, L'Aquila, Italy\\
\email{phuong.nguyen@univaq.it}\\
\url{https://www.disim.univaq.it/ThanhPhuong}
\and
%
Tien N. {\bf Nguyen}
\at Computer Science Department, University of Texas at Dallas \\
800 W. Campbell Road, ECSS 4.229 Richardson, TX 75080-3021, USA\\
\email{Tien.N.Nguyen@utdallas.edu}\\
\url{https://personal.utdallas.edu/~tien.n.nguyen}
\and
%
Nicole {\bf Novielli}
\at Dipartimento di Informatica, University of Bari ``A. Moro''\\
Via Orabona 4, 70125 Bari, Italy\\
\email{nicole.novielli@uniba.it}\\
\url{https://collab.di.uniba.it/nicole}
\and
%O
Ruben {\bf Opdebeeck}
\at Software Languages Lab, Vrije Universiteit Brussel\\
Pleinlaan 2, 1050 Elsene, Belgium\\
\email{Ruben.Denzel.Opdebeeck@vub.be}\\
\url{http://soft.vub.ac.be/soft/members/ropdebee}
\and
%P
Alfonso {\bf Pierantonio}
\at University of L'Aquila\\
Via Vetoio snc, L'Aquila, Italy\\
\email{alfonso.pierantonio@univaq.it}\\
\url{https://www.disim.univaq.it/AlfonsoPierantonio}
\and
%R
Pooya {\bf Rostami Mazrae}
\at Software Engineering Lab, University of Mons\\
Avenue Maistriau 15, 7000 Mons, Belgium\\
\email{pooya.rostamimazrae@umons.ac.be}\\
\url{https://pooya-rostami.github.io}
\and
%S
Alexander {\bf Serebrenik}
\at Eindhoven University of Technology\\
P.O. Box 513, 5600 MB Eindhoven, The Netherlands\\
 \email{a.serebrenik@tue.nl}\\
\url{https://www.win.tue.nl/~aserebre}
\and
%T
Christoph {\bf Treude}
\at School of Computing and Information Systems, University of Melbourne\\
700 Swanston Street, Carlton, Victoria, 3053, Australia\\
\email{christoph.treude@unimelb.edu.au}\\
\url{https://ctreude.ca}
\and
%W
Mairieli {\bf Wessel}
\at Institute for Computing and Information Sciences, Radboud University\\
Toernooiveld 212, 6525 EC Nijmegen, The Netherlands\\
\email{mairieli.wessel@ru.nl}\\
\url{https://mairieli.com}
\and
%X
Bowen {\bf Xu}
\at Singapore Management University\\
80 Stamford Road, Singapore 178902\\
\email{bowenxu.2017@smu.edu.sg}\\
\url{https://bowenxu.me}
\and
%Y
Zhou {\bf Yang}
\at Singapore Management University\\
80 Stamford Road, Singapore 178902\\
\email{zyang@smu.edu.sg}\\
\url{https://yangzhou6666.github.io}
\and
%Z
Stefano {\bf Zacchiroli}
\at LTCI, Télécom Paris, Institut Polytechnique de Paris\\
19 place Marguerite Perey, 91120 Palaiseau, France\\
\email{stefano.zacchiroli@telecom-paris.fr}\\
\url{https://upsilon.cc/zack}
\and
%
Ahmed {\bf Zerouali}
\at Software Languages Lab, Vrije Universiteit Brussel\\
Pleinlaan 2, 1050 Elsene, Belgium\\
\email{ahmed.zerouali@vub.be}\\
\url{http://soft.vub.ac.be/soft/members/azeroual}
\end{thecontriblist}


==> book/foreword.tex <==
%%%%%%%%%%%%%%%%%%%%%%foreword.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample foreword
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\foreword

Emacs or vi(m)? Even with the integration of Visual Studio Code (VSCode) inside GitHub, there is no end in sight for the quintessential editor wars. Since the mid '80s, thousands of online, mostly futile, discussions and flamewars have focused on which editor is the best for coding and other text processing tasks. At the surface level, this long-standing debate seems to focus merely on factors like the graphical user interface of the editors, modal vs. chord-based keyboard handling, or availability of the editors on a variety of operating systems. 

However, to actual users of these tools the choice for a given editor really is based on two key criteria: (1) the ability to customize the editor to their specific workflow via third-party, open-source extensions (or: ``plugins''); and (2) a sense of community and belonging amongst users and providers of third-party extensions. Extensibility is built into each of these editors via an underlying scripting language (from Emacs' underlying Lisp interpreter and vim's Vim script, to VSCode's TypeScript) and a dedicated plugin API. These two elements aim to seamlessly blend default functionality shared by all users (basic text manipulation) with highly custom functionality of interest to a fraction of the userbase (support for different versioning control systems, advanced text completion mechanisms, etc.). At the time of writing this foreword (March 2023), the popular MELPA package archive\footnote{\url{https://melpa.org}} (one of several archives for Emacs) lists 5,391 plugins, \url{vim.org} 5,888 vim plugins, and the VSCode Marketplace\footnote{\url{https://marketplace.visualstudio.com}} even 44,330 extensions!

These extensions do not come out of thin air, but build on each other, both in terms of technical dependencies and underlying ideas, based on strong interactions between communities of extension developers, users and enthusiasts. Dedicated fora on reddit or Stack Overflow feature thousands of enthusiasts exchanging ideas, workflow suggestions, ad hoc customizations, bug fixes and plans for future extensions. Furthermore, GitHub is rife with people sharing their personal configuration files (``emacs configuration'' resulted in 6,480 hits), or even standardizing them into official, supported distributions or variants of their editor (e.g., Doom Emacs or Prelude Emacs). Code contributed by such distributions as well as individual extensions can then be picked up by the developer community of the underlying editor, making its way into the upstream project. Apart from code contributions, artists also chime in to submit new themes or styles to tailor the visual aspects of their favourite editor.

In other words: each editor has its own {\em software ecosystem}, essentially consisting of a base technology (the editor itself), technical components (the editor extensions) depending on that technology and each other, and social interactions between each component's communities. As such, the point of the editor wars is not about choosing the ``best'' base technology, but about buying into the ``best'' editor ecosystem, where the definition of ``best'' refers to health-related measures such as the sustainability of an ecosystem, the absence of longstanding bugs, the rate of innovation as well as the degree to which the values of the ecosystem's community match with those of a given user.

In that respect, the so-called editor wars are actually not that different from ``competition'' between other ecosystems, such as mobile app frameworks and their respective app stores (\eg iOS versus Android ecosystems), programming languages with their third-party library support (e.g., Javascript's npm vs. Java's Maven Central ecosystems), open source Linux distributions (e.g., Fedora vs. Ubuntu ecosystems) or even software infrastructure technologies (e.g., Docker Hub vs. Kubernetes). In all these cases it is not about the base technology or product, it is all about the community, technical interactions and value creation surrounding these.

\bigskip
This seamlessly brings us to the topic of this book: given a software ecosystem, how can one measure and monitor its health, innovation, value, etc. in a consistent and effective manner? What kinds of data sources are available to gauge an ecosystem's development practices, evolution and internal conflicts, both amongst ecosystem contributors or between competing ecosystem projects? How can this data be obtained, cleaned and preprocessed? What kinds of analyses should be performed, and which models could be used? How to interpret the resulting findings, and how can they impact the state-of-the-practice of software ecosystems?

For one, these questions address the essential concerns practitioners have when trying to select the right ecosystem for their business, to plan maintenance activities, or to identify important health risks that might impact (parts of) their ecosystems. This is very clear from current initiatives like the Linux Foundation's CHAOSS project\footnote{\url{https://chaoss.community}}, which stands for ``Community Health Analytics in Open Source Software''. Together with industry, various CHAOSS working groups have developed a catalog of (thus far) 79 health metrics at the level of individual software projects, only 9 of which catch some aspect of health at the ecosystem level. Hence, in order to get insights in new ecosystem-level health metrics and to automate their measurement, this book is indispensable.

At the same time, researchers and students need to learn about the state-of-the-art in this domain in order to study ever more challenging software ecosystem topics. What has attracted me to this research domain, and also led me to participate in an international research project on ecosystem health with researchers of Wallonia (Belgium) and Quebec (Canada), is the need for interdisciplinary research. Research labs in sociology, biology, information sciences, etc. have developed highly sophisticated theories and metaphors that provide unique perspectives on ecosystem health. Yet, these labs lack the software engineering and software analytics backgrounds required to empirically validate such theories. Again, a book like this one prepares the reader for exactly this purpose.

Finally, what will the future bring to the domain of software ecosystems and its researchers? Similar to how software ecosystems are more than just a set of individual open source projects, ecosystems of ecosystems are more than just an agglomeration of individual ecosystems. Going back to our example ecosystem of editors, the recent breakthrough of Microsoft's Language Server Protocol (LSP) has shown ways in which innovation not only propagates from one ecosystem (VSCode) to its competing ecosystems, but also that it can spawn a new, interacting ecosystem of language servers as a side-effect. Such meta-phenomena can have disruptive side-effects on software ecosystems, hence necessitating thorough empirical research.

At the same time, it will be fascinating to understand how the role of AI will impact existing ecosystems. While, thus far, ecosystem communities consist of actual humans assisted by bots for rote automation of tedious tasks, the introduction of AI agents whose contributions might be hard to distinguish from human contributions, has the potential to disrupt or even sabotage today's ecosystem dynamics. Once more, the advent of AI in software ecosystems provides another major opportunity to validate existing theories of ecosystem dynamics using the techniques presented by this book.

\vspace{\baselineskip}
\begin{flushright}\noindent
  Kingston,\hfill {\it Bram  Adams}\\
  Ontario (Canada),\hfill (proud user of the \\
  March 2023\hfill Emacs ecosystem)
\end{flushright}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../book"
%%% End:


==> book/part0.tex <==
%%%%%%%%%%%%%%%%%%%%%part.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% sample part title
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{partbacktext}
\part{SOFTWARE ECOSYSTEM REPRESENTATIONS}
\label{part:representing}

\end{partbacktext}

==> book/part1.tex <==
%%%%%%%%%%%%%%%%%%%%%part.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% sample part title
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{partbacktext}
\part{ANALYSING SOFTWARE ECOSYSTEMS}
\label{part:analysing}

\end{partbacktext}

==> book/part2.tex <==
%%%%%%%%%%%%%%%%%%%%%part.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% sample part title
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{partbacktext}
\part{EVOLUTION WITHIN SOFTWARE ECOSYSTEMS}
\label{part:evolution}

\end{partbacktext}

==> book/part3.tex <==
%%%%%%%%%%%%%%%%%%%%%part.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% sample part title
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{partbacktext}
\part{SOFTWARE AUTOMATION ECOSYSTEMS}
\label{part:process}


\end{partbacktext}

==> book/part4.tex <==
%%%%%%%%%%%%%%%%%%%%%part.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% sample part title
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{partbacktext}
\part{MODEL-CENTERED SOFTWARE ECOSYSTEMS}
\label{part:models}

\end{partbacktext}

==> book/preface.tex <==

\preface


The discipline of \emph{software engineering} emerged in 1969 as a result from the first international conference on software engineering that took place in Garmisch ( Germany), and that was sponsored by the NATO Science Committee. %\cite{Naur1969}.\tom{Citation removed since not allowed in preface...}
Over a period spanning several decades, the discipline has given rise to increasingly advanced processes and tool support for maintaining and evolving ever more complex and interconnected software products.
Software engineering tools offer support for a wide range of activities including project management, version control, configuration management, collaborative coding, quality assurance, dependency management, continuous integration and deployment, containerisation and virtualisation.

Since the seminal book ``Software Ecosystem" by Messerschmitt and Szyperski in 2003, %\cite{messerschmitt2003software}\tom{Citation removed since not allowed in preface...}
\emph{software ecosystems} have become a very active topic of research in software engineering. 
As the different chapters of this book will reveal, software ecosystems exist in many different forms and flavours, so it is difficult to provide a unique encompassing definition.
 But a key aspect of such software ecosystems is that software products can no longer be considered or maintained in isolation, since they belong to ever more interconnected and interdependent networks of co-evolving software components and systems.
This was enabled by technological advances in various domains such as component-based software engineering, global software development and cloud computing. 
The ever increasing importance of collaborative online ``social'' coding platforms, %\cite{Dabbish2012}, \tom{Citation removed since not allowed in preface...}
aiming to develop software in a collaborative way, has made software ecosystems indispensable to software practitioners, in commercial as well as open source settings.
This has lead to the widespread use and popularity of large registries of reusable software libraries for a wide variety of programming languages, operating systems and project-specific software communities.



\paragraph{\textbf{How this book originated}}

The idea to write this book originated from a large inter-university fundamental research project ---called SECOAssist (see \url{secoassist.github.io})--- that studied the technical aspects of software ecosystems, in order to provide tools and techniques to assist contributors, maintainers, managers and other ecosystems stakeholders in their daily activities. This project was financed by the Belgian regional science foundations F.R.S.-FNRS and FWO-Vlaanderen under the ``Excellence of Science'' seal. It took place from 2018 till 2023 and spawned many research results in the form of scientific publications, PhD dissertations, open source tools and datasets. The three co-editors of this book, Tom Mens, Coen De Roover and Anthony Cleve, were principal investigators of the project together with Serge Demeyer, leading the research efforts of their respective teams.

The conducted research was quite diverse, covering a wide range of software ecosystems and focussing on challenging technical and socio-technical aspects thereof.
Among others, we empirically analysed a wide range of maintenance issues related to software ecosystems of reusable software libraries. % (such as npm for JavaScript, Maven for Java, RubyGems for Ruby, Packagist for PHP, CRAN for R, CPAN for Perl, NuGet for .NET).
Example maintenance issues studied include outdatedness, security vulnerabilities, semantic versioning, how to select, replace and migrate software libraries, and contributor abandonment.
We also investigated advanced testing techniques such as test amplification and test transplantation and how to apply them at the ecosystem level.
We studied socio-technical aspects in the \github ecosystem, including the phenomenon of forking, the use of development bots and the integrated CI/CD workflow infrastructure of \github Actions.
We also analysed issues around database usage and migration in ecosystems for data-intensive software.
Finally, we explored maintenance issues in a range of emerging software ecosystems, such as the \dockerhub containerisation ecosystem, the Intrastructure-as-Code ecosystem forming around \ansible Galaxy, the Q\&A ecosystem of \stackoverflow, the \openstack ecosystem, and the \actions ecosystem.

\paragraph{\textbf{Who contributed to this book}}

This book aims to further expand upon and report about the software ecosystems research that has been conducted in recent years, going well beyond the results achieved by the SECOAssist research project.
To this end, we invited some of the most renowned researchers worldwide who have made significant contributions to the field.
Their names and affiliations can be found just before the book's table of contents.
The chapters they have contributed focus on the nature of particular software ecosystems, or on specific domain-specific tooling and analyses to understand, support, and improve those ecosystems.

Following the spirit of open science and collaborative development practices, we used a GitHub repository during the process of writing and reviewing the book chapter. Each contributor had access to the material of each chapter, and each chapter was peer-reviewed by at least three different contributors using the repository's discussion forum.

\paragraph{\textbf{What this book IS NOT about}}

Previously published books on the topic of software ecosystems have primarily focused on the business aspects of software ecosystems:
%\cite{messerschmitt2003software,Popp2010,Jansen2013book}.\tom{removed citations since not allowed in preface}
\begin{itemize}
\item D.G. Messerschmitt, C. Szyperski (2003) Software ecosystem: Understanding an indispensable technology and industry. MIT press
\item K.M. Popp, R. Meyer (2010) Profit from Software Ecosystems: Business Models, Ecosystems and Partnerships in the Software Industry. Norderstedt, Germany 
\item S. Jansen, S. Brinkkemper, M.A. Cusumano (2013) Software Ecosystems: Analyzing and Managing Business Networks in the Software Industry. Edward Elgar Publishing
\end{itemize}
We fully agree these are very important aspects, but regretted the absence of a complementary book focusing on the technical aspects related to empirically analysing, supporting, and improving software ecosystems.
This is the main reason why we decided to create this book.

Even though we have tried to be as comprehensive as possible, we acknowledge that this book might not cover all important research topics related to software ecosystems. We apologise to the reader if specific technical or other aspects related to software ecosystems and their analysis have not been sufficiently addressed.

\paragraph{\textbf{Who this book is intended for}}

This book is intended for all those practitioners and researchers interested in developing tool support for or in the empirical analysis of software ecosystems. The reader will find the contributed chapters to cover a wide spectrum of social and technical aspects of software ecosystems, each including an overview of the state of the art.

While this book has not been written as a classical textbook, we believe that it can be used as supplementary material to present software ecosystems research during advanced (graduate or postgraduate) software engineering lectures and capita selecta. This is exactly what we, book editors, intend to do as well in our own university courses.
For researchers, the book can be used as a starting point for exploring the wealth of software ecosystems results surveyed in each chapter.

\paragraph{\textbf{How this book is structured}}

This book starts with an introductory chapter (\chap{INT}) that provides a historical account of the origins of software ecosystems. This chapter sets the necessary context about the domain of software ecosystems by highlighting its different perspectives, definitions and representations. It also provides many concrete examples highlighting the variety of software ecosystems that have emerged during the previous decades.

The book is composed of five parts, each containing two contributed chapters.
Part~\ref{part:representing} contains three chapters on software ecosystem representations. 
\chap{SWH} focuses on the Software Heritage open science ecosystem. This ecosystem has been recognised by UNESCO because of its ongoing effort to preserve and provide access to the digital heritage of free and open source software. The chapter focuses on important aspects such as open science and research reproducibility, and also discusses some of the techniques that are required to maintain and query this massive software ecosystem.
\chap{PPM} reflects on software ecosystems composed of many interdependent components, and the challenges that researchers are facing to mine such ecosystems. The authors propose a list of promises and perils related to these challenges.

Part~\ref{part:analysing} of the book contains two chapters that focus on different ways and techniques of analysing software ecosystems.
\chap{SLU} focuses on technical aspects of how to mine software library usage patterns in ecosystems of reusable software libraries.
\chap{EMO} focuses on social aspects in software ecosystems, by analysing how emotions play a role in the context of developer communication and interaction. It presents a range of sentiment analysis techniques and tools that can be used to carry out such analyses.

Part \ref{part:evolution} of the book contains two chapters that focus on aspects related to the evolution of software ecosystems.
\chap{FRK} focuses on the phenomenon of \emph{forking} of software repositories in social coding ecosystems such as \github. The chapter studies the prevalent phenomenon of variant forks as a reuse mechanism to split of software projects and steer them into a new direction. The focus is on how such variant forks continue to be maintained over time and to which extent they co-evolve with the main repository they originated from.
\chap{COL} discusses the effect of \emph{collateral evolution} in software ecosystems. Collateral evolution is a type of adaptive maintenance %\cite{LientzSwanson1980,Chapin2001}\tom{Removed citations since not allowed to have them in preface.}
that is required to keep a software system functional when its surrounding technological environment is facing changes that are beyond the control of the system itself. A typical example of this are external libraries that subject to frequent changes that often require the software system to adapt to them. This phenomenon is explored for three software ecosystems (the Linux kernel, Android apps, and machine learning software), and techniques are presented to support collateral evolution in those ecosystems.


Part~\ref{part:process} of the book looks at what could be called software automation ecosystems. Such ecosystems are brought about by the increasing automation of software engineering processes. \chap{WFA} studies development workflow automation tools, considering the \github Actions ecosystems and the use of development bots.
\chap{IAC} looks at the ecosystems that have formed around containerisation and configuration management tools, focusing specifically on the \dockerhub and Ansible Galaxy ecosystems.

Finally, Part~\ref{part:models} focuses on what could be called model-centered software ecosystems.
\chap{MDE} considers ecosystems stemming from \emph{model-driven software engineering}. Such ecosystems contain software model artefacts and associated tools. The chapter focuses on how machine learning and deep learning techniques can be used to understand and analyse the artefacts contained in such ecosystems.
Last but not least, \chap{DIS} looks at \emph{data-intensive software ecosystems}, which are ecosystems in which database models and their corresponding tools form a crucial role. The chapter focuses on techniques to mine, analyse sand visualise such ecosystems. It also reports on empirical analysis based on such techniques.

\paragraph{\textbf{Acknowledgments}}
We thank the FWO-Vlaanderen and F.R.S-FNRS Science Foundations in Belgium for the generous research funding they have provided to us for our research on software ecosystems. We also thank our respective universities in Mons, Brussels, and Namur for having given us the opportunity, environment and resources to carry out our research and to enable this research collaboration. We express our gratitude to all chapter authors of this book for having taken the time and effort to contribute high-quality chapters while respecting the imposed deadlines. Last but not least, we thank our loving families friends and colleagues for their support.

\vspace{\baselineskip}
\begin{flushright}\noindent
    Belgium,\hfill {\it Tom  Mens, University of Mons}\\
    March 2023\hfill {\it Coen  De Roover, Vrije Universiteit Brussel}\\
    \hfill {\it Anthony  Cleve, University of Namur}\\

\end{flushright}




==> book/title.tex <==
%%%%%%%%%%%%%%%%%%%%%part.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% sample part title
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{partbacktext}
\part*{Software Ecosystems:\\ Tooling and Analytics}
\label{part:title}

{\Large Preprint of  a book, to be published by Springer.}

\smallskip
{\large Date of generation of this document: \today}

\bigskip
{\huge Editors}

\smallskip
{\LARGE Tom Mens $\cdot$ Coen De Roover $\cdot$ Anthony Cleve}


\end{partbacktext}
